Federated Clustering: An Unsupervised Cluster-Wise Training for Decentralized Data Distributions

Federated Learning (FL) enables decentralized machine learning while preserving data privacy, making it ideal for sensitive applications where data cannot be shared. While FL has been widely studied in supervised contexts, its application to unsupervised learning remains underdeveloped. This work introduces FedCRef, a novel unsupervised federated learning method designed to uncover all underlying data distributions across decentralized clients without requiring labels. This task, known as Federated Clustering, presents challenges due to heterogeneous, non-uniform data distributions and the lack of centralized coordination. Unlike previous methods that assume a one-cluster-per-client setup or require prior knowledge of the number of clusters, FedCRef generalizes to multi-cluster-per-client scenarios. Clients iteratively refine their data partitions while discovering all distinct distributions in the system. The process combines local clustering, model exchange and evaluation via reconstruction error analysis, and collaborative refinement within federated groups of similar distributions to enhance clustering accuracy. Extensive evaluations on four public datasets (EMNIST, KMNIST, Fashion-MNIST and KMNIST49) show that FedCRef successfully identifies true global data distributions, achieving an average local accuracy of up to 95%. The method is also robust to noisy conditions, scalable, and lightweight, making it suitable for resource-constrained edge devices.

==> z_02_OLD.tex <==
\subsection*{Phase 5: System Convergence and Stopping Conditions}

After clients refine their local clusters using the federated models, the stopping conditions are evaluated before initiating a new iteration (line~\ref{alg1:line:convergence} of Algorithm~\ref{alg:fed_complete}). These conditions are assessed based on the system state at the end of each iteration to determine whether further refinement is necessary.

\textit{Client-level Clustering Stability Check:}
%This process involves comparing the cluster labels from previous and current iterations within each client. We define the set of active clients in any iteration as $A$. An active client is one whose local clustering has not yet reached a state of stability based on a chosen metric.
This process involves tracking the evolution of cluster assignments across iterations for each client. A client is considered stable if its updated local clustering exhibits no \textit{significant deviation} from the previous iteration.
% 
Since clustering algorithms assign arbitrary labels, direct element-wise comparison of cluster assignments is not meaningful.
Just as an illustration example, consider a client $C_i$ that labels its clusters numerically from $1$ to $K_i$. Suppose that in round $t$, data points from an unknown distribution $U_l$ are assigned to cluster $j$, and in round $t+1$, those same points are instead assigned to cluster $w$. Although the points remain grouped consistently, the cluster label has changed. In the absence of ground-truth labels, the system must infer such correspondences by comparing the cluster assignments of data points across consecutive rounds.
% 
To address this, Clustering Accuracy (ACC) is used, which first determines the optimal label correspondence before computing the accuracy.
While ACC is commonly used to evaluate clustering results against ground-truth labels when available~\citep{xie2016unsupervised}, it can also be applied more generally to measure the agreement between two different clustering assignments $y$ and $y'$: 

\begin{equation}
\text{ACC}(y', y) = \max_{\pi \in \Pi} \frac{1}{n} \sum_{i=1}^n 1\{ y'_i = \pi(y_i) \}
\label{eq:acc}
\end{equation}


Here,  $\Pi$  represents the set of all possible label permutations. The goal is to find the permutation $\pi$  that maximizes the agreement between cluster assignments. Instead of exhaustively checking all permutations, the Hungarian algorithm~\citep{Kuhn1955Mar} efficiently finds the optimal label permutation $\pi$ in polynomial time.
For instance, with $y' = [0, 0, 1, 1, 2]$ and $y = [2, 2, 1, 1, 0]$, direct comparison yields only 2/5 matches, but with optimal permutation $\pi(0)=2, \pi(1)=1, \pi(2)=0$, ACC = 1.0, confirming identical groupings despite different labels.


In our context, we define active clients (set $A$)  as those whose local clustering hasn't yet stabilized according to this metric. Specifically, the ACC is evaluated between the previous ($y'$) and current ($y$) cluster labels for each specific client $C_i$:

\begin{equation*}
    A = \{C_i: \text{ACC}( y'_{C_i}, y_{C_i}) < \tau ~ \forall C_i \in C \}
\end{equation*}

A client is removed from the active set $A$ if its ACC exceeds a predefined threshold $\tau$. When the ACC is higher than $\tau$, the difference between two iterations' clustering is minimal, suggesting that the client's clusters have stabilized.


Clients that have reached this stability level, referred to as \emph{non-active} clients, must still participate in the federated learning process. In fact, while they stop further training of their local models and refining their clusters (lines~\ref{alg1:line:local_train} and \ref{alg1:line:cluster_refine} of Algorithm~\ref{alg:fed_complete}), they remain actively engaged in Step 2, i.e., continuing to exchange models and establish associations with other participants.
This ongoing participation is crucial for maintaining the stability of the process, as it ensures that stabilized clients continue contributing their associated samples to the federated process.


On the other hand, clients that have stabilized but retain incorrect data partitioning (i.e., misaligned with the true categories) also remain actively engaged in Step 2. However, they are less likely to establish new associations, which naturally limits the propagation of misaligned clusters and helps preserve the integrity of the global process.


\textit{Global-level Stop Condition:} In addition to the other condition, based on the active clients in the process, we monitor the trends in the number of isolated clusters $|I|$ and the formation of communities $G$ within the system. The process is halted if these metrics remain stable over a predetermined number of iterations, indicating no significant changes. In our experiment, we specifically use the criteria that when both the number of communities and the number of isolated clusters do not change by more than 10\% over three consecutive iterations, the process is stopped. This ensures that the process halts when further iterations are unlikely to yield significant changes.


In summary, the iterative federated learning process takes into account both the stability of individual clients and the overall system metrics. The process concludes either when there are no more active clients remaining in set $A$, or when the global stopping condition is satisfied.



